U Can't Gen This? A Survey of Intellectual Property Protection Methods for Data in Generative AI

Large Generative AI (GAI) models have the unparalleled ability to generate text, images, audio, and other forms of media that are increasingly indistinguishable from human-generated content. As these models often train on publicly available data, including copyrighted materials, art and other creative works, they inadvertently risk violating copyright and misappropriation of intellectual property (IP). Due to the rapid development of generative AI technology and pressing ethical considerations from stakeholders, protective mechanisms and techniques are emerging at a high pace but lack systematisation. In this paper, we study the concerns regarding the intellectual property rights of training data and specifically focus on the properties of generative models that enable misuse leading to potential IP violations. Then we propose a taxonomy that leads to a systematic review of technical solutions for safeguarding the data from intellectual property violations in GAI.

==> overview.tex <==
\begin{table*}[ht]
    \caption{An overview and taxonomy of mitigation techniques for IPR protection in generative AI}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|l|l|l}
        \toprule
         \textbf{Approach}& \textbf{Domain} & \textbf{IPR violation type} & \textbf{Phase of application}  \\
         \midrule
         Deduplicating training data\cite{carlini_extracting_2023} & all & data replication & training time  \\
         Image caption modification\cite{somepalli_understanding_2023} & text-to-image & data replication & training/inference time  \\
         Machine Unlearning\cite{sekhari_remember_2021,neel_descent--delete_2020,zhang_forget-me-not_2023,golatkar_eternal_2020} & all & data replication & training time \\
         Cloaking\cite{shan_glaze_2023} & text-to-image & mimicry & training/fine-tuning\\
        Concept removal&&&\\
         \hspace{10pt} Safe latent diffusion\cite{schramowski_safe_2023} & text-to-image  & mimicry & inference time\\
          \hspace{10pt} Erasing concepts \cite{gandikota_erasing_2023} & text-to-image & mimicry & fine-tuning\\
          \hspace{10pt} Concept ablation \cite{kumari_ablating_2023} & text-to-image & replication, mimicry & fine-tuning\\
          \hspace{10pt} Data redaction\cite{kong_data_2023} & GANs & mimicry & training \\
         Spawning\cite{noauthor_spawningai_nodate}& any & replication, mimicry & - \\
         Consent-respecting training\cite{noauthor_holly_nodate} & any & mimicry & training time \\
         Testing memorisation\cite{carlini_secret_2019} & text models & replication & training time \\
         \bottomrule
    \end{tabular}
    }
    \label{tab:mitigation}
\end{table*}
